Modularity of nearly ordinary 2-adic residually dihedral Galois representations

We prove modularity of some two dimensional, 2-adic Galois representations over totally real fields that are nearly ordinary and that are residually dihedral. We do this by employing the strategy of Skinner and Wiles, using Hida families, together with the 2-adic patching method of Khare and Wintenberger. As an application we deduce modularity of some elliptic curves over totally real fields that have good ordinary or multiplicative reduction at places above 2.

==> MainThms/OldExamples.tex <==
We show how the main theorem implies the corollary from the introduction and conclude by giving some examples of elliptic curves satisfying the assumptions of the corollary from the introduction. For any finite place $v$ of $F$, we normalize the valuation $\val_v$ at $v$ so that a uniformizer has valuation $1$.

\subsubsection{Proof of the main corollary}\label{MainCorProof}

Let $E$ be an elliptic curve over $F$ given by the the Weierstrass equation
	\[ y^2 = x^3 + ax + b.
	\]
The curve $E$ has $2$-torsion defined over $F$ if and only if $x^3 + ax + b$ is reducible. Further, the $G_F$-representation $E[2](\Qbar)$ is absolutely irreducible if and only if the splitting field of $x^3 + ax +b$ is an $S_3$-extension, which happens if and only if $x^3+ax+b$ is irreducible and the discriminant 
	\[\Delta = -16(4a^3 + 27b^2)
	\]
of the Weierstrass equation is not a square in $F$. Note $\Delta$ differs from the discriminant $\Delta_E$ of $E$ by a square; so, $\Delta$ is not a square if and only if $\Delta_E$ is not a square. If the action of $G_F$ on $E[2](\Qbar)$ is absolutely irreducible, then the unique quadratic extension $L/F$ for which the action of $G_L$ on $E[2](\Qbar)$ is abelian is $F(\sqrt{\Delta})$. Lastly, $E$ has multiplicative reduction at $v|2$ if and only if $j_E$ is non-integral at $v$, and has potentially ordinary reduction if and only if $j_E$ is a unit at $v$, c.f. \cite{SilvermanEllCurves}*{Chapter V, Exercise 5.7}. The corollary now follows from the main theorem. \hfill \qed

Note that any elliptic curve satisfying our assumptions is not CM. If it were, then there would be a quadratic CM extension $L/F$ such that the representation $\rho_E|_{G_L}$ is abelian.  By the absolute irreducibility of $E[2](\Qbar)$, we have $L = F(\sqrt{\Delta})$, and $\Delta$ is totally negative. The reducibility of $\rho_E|_{G_v}$ for each $v|2$ then implies that every $v|2$ splits in $F(\sqrt{\Delta})$, a contradiction.

\subsubsection{An example}\label{TheExamples}

We give an explicit infinite family of elliptic curves $E_\alpha$ over $F$ satisfying the assumptions of the corollary. Take $\alpha \in F$ such that
\begin{enumerate}
	\item[(a)] $\mathrm{val}_v(\alpha) \ge 6 \val_v(2)$ for all $v|2$;
	\item[(b)] there is some $w_0|3$ such that $\val_{w_0}(2+\alpha) = 1$;
	\item[(c)] either 
	\begin{itemize}
		\item[-] there is some finite place $w\nmid 3$ such that $\val_w(\alpha)$ is $\ge 0$ and odd, or
		\item[-] there is some $\sigma: F \hookrightarrow \R$ such that either $\sigma(\alpha)< -4$ or $\sigma(\alpha) > 0$;	
	\end{itemize}
		\item[(d)] either
		\begin{itemize}
		\item[-] there is some $\sigma_0: F\hookrightarrow \R$ such that $-4 < \sigma_0(\alpha) < 0$, or
		\item[-] there is some $v_0|2$ such that $\mathrm{val}_{v_0}(\alpha)$ is odd.
	\end{itemize}
\end{enumerate}

Let $E_\alpha$ by the elliptic curve given by the Weierstrass equation
	\[ y^2 = x^3 - 3x + 2 + \alpha.
	\]
The discriminant (of the Weierstrass equation) and the $j$-invariant are given by
	\[ \Delta = -16\cdot 27\alpha(4+\alpha) \hspace{0.5cm} \text{and} \hspace{0.5cm}
	 j = \frac{2^8\cdot 3^3}{\alpha(4+\alpha)},
	\]
respectively. For any $v|2$, since $\val_v(\alpha) \ge 6 \val_v(2)$ by (a), we have $\val_v(4+\alpha) = \val_v(4) = 2\val_v(2)$ and
	\[ \val_v(j) = 8\val_v(2) - 2\val_v(2) - \val_v(\alpha) \le 0.
	\]
By (b), there is some $w_0|3$ such that $\val_{w_0}(2+\alpha) = 1$. This implies that polynomial $x^3 + 3x + (2+\alpha)$ is irreducible, by the Eisenstein criterion. 

If there is $v_0|2$ such that $\val_{v_0}(\alpha)$ is odd, then $\val_{v_0}(4+\alpha) = \val_{v_0}(4)$ and 
	\[
	\val_{v_0}(\Delta) = \val_{v_0}(-16\cdot 27 \alpha (4+\alpha)) = 6\val_{v_0}(2) + \val_{v_0}(\alpha)
	\]
is odd. This implies $\Delta$ is not a square in $F_{v_0}$. In particular, it is also not a square in $F$. Otherwise, assumption (d) implies that 
	\[
	\sigma_0(\Delta) = \sigma_0(-16\cdot 27\alpha(4+\alpha)) > 0.
	\]
So, $\Delta$ is not totally negative. It remains to check in this case that $\Delta$ is not a square in $F$. Assumption (c) implies that either there is some $w\nmid 3$ such that $\val_w(\alpha)$ is $\ge 0$ and odd, or there is some $\sigma:F \hookrightarrow \R$ such that $\sigma(\alpha) \notin [-4,0]$. Assume we are in the first case. If $w|2$, it was shown above that $\Delta$ is not a square in $F_w$; in particular, it is not a square in $F$. If $w\nmid 6$, then $-16\cdot 27(4+\alpha)$ is a unit in $F_w$ and $\val_w(\Delta)$ is odd. Then, $\Delta$ is not a square in $F_w$; in particular, it is not a square in $F$. In the second case, $\sigma(\Delta) < 0$, and is not a square under $\sigma$; in particular, it is not a square in $F$. 

By weak approximation, there are infinitely many $\alpha \in F$ satisfying (a), (b), either of the conditions of (c), and either of the conditions in (d). If $\alpha$ satisfies $(a)$, then $-4-\alpha$ does not, and the map $\alpha \mapsto j = \frac{2^8\cdot 3^3}{\alpha(4+\alpha)}$ is one-to-one. This gives an infinitely many non-isomorphic, non-CM elliptic curves satisfying the assumptions of the corollary.

==> prelim.tex <==
%Preliminary pages

\title{Modularity of nearly ordinary $2$-adic residually dihedral Galois representations}

\author{Patrick Brodie Allen}
\department{Mathematics}
\degreeyear{2012}

\chair{Chandrashekhar Khare}
\member{Haruzo Hida}
\member{Don Blasius}
\member{Amit Sahai}

\dedication{To my father and mother, David and Michele, and my brothers, Kyle, Aaron, and Sean}

\acknowledgments{I would like to thank my advisor Professor Chandrashekhar Khare for suggesting to me this problem and for his patience and guidance throughout its resolution. I would like to thank the entire number theory group at UCLA for providing a stimulating place to learn and work. I would like to thank Mark Kisin and Gebhard B\"{o}ckle for helpful conversations. I would like to thank David Geraghty for helpful conversations and correspondence regarding ordinary deformation rings and Andrew Snowden for helpful correspondence regarding his work. Lastly I would like to thank Anush Tserunyan for unbounded moral support and constant encouragement.}

\vitaitem{2003--2004}{Undergraduate Teaching Assistant, Faculty of Mathematics, University of Waterloo}
\vitaitem{2004}{BMath in Pure Mathematics, University of Waterloo}
\vitaitem{2004--2006}{Teaching Assistant, Faculty of Mathematics, University of Waterloo}
\vitaitem{2006}{MMath in Pure Mathematics, University of Waterloo}
\vitaitem{2006--present}{Teaching Assistant, Department of Mathematics, UCLA}
\vitaitem{2010}{Vigre Graduate Student Instructor, Department of Mathematics, UCLA}

\publication{Patrick B. Allen, \textit{On the multiplicity of linear recurrence sequences}, J. Number Theory 126 (2007), no. 2, 212-216}

\abstract{We prove modularity of some two dimensional $2$-adic Galois representations over a totally real field that are nearly ordinary at all places above $2$ and that are residually dihedral. We do this by employing the strategy of Skinner and Wiles using Hida families together with the $2$-adic patching method of Khare and Wintenberger. As an application we deduce modularity of some elliptic curves over totally real fields that have good ordinary or multiplicative reduction at places above $2$.}
